Multiview Transformers for Video Recognition

Video understanding requires reasoning at multiple spatiotemporal resolutions -- from short fine-grained motions to events taking place over longer durations. Although transformer architectures have recently advanced the state-of-the-art, they have not explicitly modelled different spatiotemporal resolutions. To this end, we present Multiview Transformers for Video Recognition (MTV). Our model consists of separate encoders to represent different views of the input video with lateral connections to fuse information across views. We present thorough ablation studies of our model and show that MTV consistently performs better than single-view counterparts in terms of accuracy and computational cost across a range of model sizes. Furthermore, we achieve state-of-the-art results on six standard datasets, and improve even further with large-scale pretraining. Code and checkpoints are available at: https://github.com/google-research/scenic/tree/main/scenic/projects/mtv.

==> fusion_layers.tex <==

\begin{table} 
	\centering
	\scriptsize{
\begin{tabular}{  c  c  c  c }
    \toprule
    Fusion layers & GFLOPs & MParams & Top-1 \\
    \midrule
    Late fusion & 168 & 231 & 79.22 \\
    \midrule
    0 & \multirow{3}{*}{195} & \multirow{3}{*}{314} &  80.96 \\
    5 & &  & 81.08 \\
    11 & &  & 81.00 \\ \midrule
    0, 1 & \multirow{4}{*}{203} & \multirow{4}{*}{323} & 80.91 \\
    5, 6 &  &  & 80.96 \\
    10, 11 &  &  & 80.81 \\
    5, 11 &  & & \textbf{81.14} \\
    \midrule
    0, 5, 11 & 210 & 331 & 80.95 \\
    \bottomrule
   \end{tabular}
   }
	\caption{Effects of applying CVA at different layers. Late fusion is used as the baseline for comparison, and the model variant used in this study is B/4+S/8+Ti/16. All ``Base'', ``Small'', and ``Tiny'' models have 12 layers.}
\label{tab:cva_layers}
\end{table}


==> slowfast.tex <==

\begin{table} 
	\centering
	\scriptsize{
\begin{tabular}{  l  c  c  c }
    \toprule
    Model variants & GFLOPs & MParams & Top-1 \\
    \midrule
    \multicolumn{3}{l}{\textit{SlowFast multi-view method}} \\
    $\text{B}_{4\times16}$ (Slow-only) & 79 & 87 & 78.0 \\
    $\text{Ti}_{16\times4}$ (Fast-only) & 63 & 6 & 74.6 \\
    $\text{B}_{4\times16}+\text{Ti}_{16\times4}$ & 202 & 105 & 79.7 \\ \midrule
    B/4+Ti/16 (ours) & 168 & 224  & \textbf{80.8} \\
    \bottomrule
   \end{tabular}
   }
	\caption{Comparison between MTV and the SlowFast method with a transformer backbone. For SlowFast's inputs, $x \times y$ denotes $x$ number of frames sampled at a temporal stride $y$. Our method is more accurate while using less FLOPs.}
\label{tab:slowfast}
\end{table}

